Subspace Differential Privacy

Many data applications have certain invariant constraints due to practical needs. Data curators who employ differential privacy need to respect such constraints on the sanitized data product as a primary utility requirement. Invariants challenge the formulation, implementation, and interpretation of privacy guarantees. We propose subspace differential privacy, to honestly characterize the dependence of the sanitized output on confidential aspects of the data. We discuss two design frameworks that convert well-known differentially private mechanisms, such as the Gaussian and the Laplace mechanisms, to subspace differentially private ones that respect the invariants specified by the curator. For linear queries, we discuss the design of near-optimal mechanisms that minimize the mean squared error. Subspace differentially private mechanisms rid the need for post-processing due to invariants, preserve transparency and statistical intelligibility of the output, and can be suitable for distributed implementation. We showcase the proposed mechanisms on the 2020 Census Disclosure Avoidance demonstration data, and a spatio-temporal dataset of mobile access point connections on a large university campus.

==> Constrained Data Privatization with Gaussian Mechanism/sections/abstract.tex <==

Many data applications have certain invariant constraints due to practical needs. Data curators who employ differential privacy need to respect such constraints on the sanitized data product as a primary utility requirement. Invariants challenge the formulation, implementation and interpretation of privacy guarantees. We propose \emph{subspace differential privacy}, to honestly characterize the dependence of the sanitized output on confidential aspects of the data. We discuss two design frameworks that convert well-known differentially private mechanisms, such as the Gaussian and the Laplace mechanisms, to subspace differentially private ones that respect the invariants specified by the curator. For linear queries, we discuss the design of near optimal mechanisms that minimize the mean squared error. Subspace differentially private mechanisms rid the need for post-processing due to invariants, preserve transparency and statistical intelligibility of the output, and can be suitable for distributed implementation. We showcase the proposed mechanisms on the 2020 Census Disclosure Avoidance demonstration data, and a spatio-temporal dataset of mobile access point connections on a large university campus.

% \robin{optimal correlated gaussian...evaluated on Census demonstration and mobility data, and distributed privatization}
% are preserved, facilitating principled downstream statistical analysis. 

==> Constrained Data Privatization with Gaussian Mechanism/sections/body.tex <==


\section{Introduction}\label{sec:intro}

% {\color{red} Title brainstorm:
% \begin{itemize}
%     \item Truth-Constrained Differential Privacy
%     \item Subspace Differential Privacy
% \end{itemize}

% }

%\robin{Can we make all citations appear as numbers? Or does that violate the AAAI format?}\fang{After some search, I think we cannot change this.}

\noindent\textbf{Invariants: a  challenge for data privacy}
Data publication that satisfies differential privacy carries the formal mathematical guarantee that an adversary cannot effectively tell the difference, in the probabilistic sense, when two databases differ in only one entry. %\fang{we are using bounded differential privacy, so we may change the framing}\jie{fixed it} 
The extent of privacy protection under differential privacy is quantified by the privacy loss budget parameters, such as in $\epsilon$-differential privacy and $(\epsilon, \delta)$-differential privacy \citep{dwork2006calibrating}.
%The utility of the sanitized data products may be evaluated in specific use cases using loss metrics on the inferential target such as bias, variance, mean squared error and so on, as functions of the privacy loss budget, hence providing potential of systematic assessment of the privacy-utility trade-off.
While the differential privacy guarantee is rigorously formulated with the probability language, its construction does not naturally mingle with hard and truthful constraints,  called \emph{invariants} \cite{ashmead2019effective},  that need to be imposed onto the sanitized data product, often as a primary utility requirement.

An important use case in which the challenge for privacy arises from invariants is the new Disclosure Avoidance System (DAS) of the 2020 Decennial Census \cite{abowd2018us}. The new DAS tabulates noise-infused, differentially private counts into multi-way contingency tables at various geographic resolutions, from the aggregated state and county levels to specific Census blocks. Due to the Census Bureau's constitutional mandate and its responsibilities as the official statistics agency of the United States, all data products must be preserved in such a way that certain aspects of their values are \emph{exactly} as enumerated. These invariants include (and are not limited to) population totals at the state level, counts of total housing units, as well as other group quarter facilities at the block level. Straightforward tabulations of the noisy measurements are most likely inconsistent with the mandated invariants. 

A common method to impose invariants on a differentially private noisy query is via post-processing using distance minimization \cite{abowd2019census,ashmead2019effective}.
%\fang{do we have more reference?}\jie{I added [1], maybe we can also add one sentence to explain what is "distance minimization"?}
 The resulting query is the solution to an optimization task, one that minimizes a pre-specified distance between the unconstrained query and the invariant-compliant space.  There are two major drawbacks to this approach. First, post-processing may introduce systematic bias into the query output. Particularly troubling is that the source of such bias is poorly understood \cite{DBLP:journals/corr/abs-2010-04327}, in part due to the highly data-dependent nature of the post-processing procedure, and the lack of a transparent probabilistic description. The TopDown algorithm \cite{abowd2019census}, employed by the Census DAS to impose invariants on the noisy measurements, exhibits a notable bias that it tends to associate larger counts with positive errors, whereas smaller counts with negative errors, when the total count is held as invariant. Figure~\ref{fig:census_trend} illustrates this phenomenon using the November 2020 vintage Census demonstration data \cite{ipums2020das}. For all states and state-level territories with more than five counties   (i.e. excluding D.C., Delaware, Hawaii and Rhode Island), a simple regression is performed between the county-level DAS errors and the log true county population sizes. Of the 48 regressions, 37 result in a negative slope estimate, out of which 11 are statistically significant at $\alpha = 0.01$ level (red circles in the left panel), indicating a systematic negative association between the DAS errors and the true counts. The bias trend is clearly visible in the right panel among the DAS errors (red squares) associated with the counties of Illinois, ordered by increasing population size. As \citet{DBLP:journals/corr/abs-2010-04327} discussed, the bias exhibited in the demonstration data is attributed to the non-negativity constraints imposed on the privatized counts.
 
 %\fang{Reviewer suggest \cite{DBLP:journals/corr/abs-2010-04327} as a related work}
 %{\color{blue} In Figure~\ref{fig:census_trend}, the proposed projected Laplace mechanism generates unbiased privacy errors (the boxplots) while respecting the state total invariant. } \robin{I added this sentence but don't know if I like it. What do you think?}\jie{I like it but for the benefit of space, maybe we skip this and only keep in the caption.}

The second, and more fundamental, drawback is that imposing invariants that are true aspects of the confidential data may incur additional privacy leakage, even if the invariants are also publicly released \cite{gong2020congenial}. When conveyed to data users and contributors, the narrative that the invariants are imposed by ``post-processing'' may lend to the erroneous interpretation that no additional leakage would occur. Care needs to be taken to explain that whenever nontrivial invariants are observed, the usual  $(\epsilon,\delta)$-differential privacy guarantee cannot be understood in its fullest sense.

%\robin{other examples where truth constraints are a problem.}

The need to impose invariants arises in application areas involving the monitoring of stochastic events in structured spatio-temporal databases.
In some cases, there are requirements to report accurate counts (service requests \cite{nyc2021} or traffic volumes \cite{sui2016characterizing,yang2019revisiting,yang2020lbsn2vec,wang2020distributed}). In other cases, there are invariants that can be derived from external common sense knowledge --e.g., the number of vehicles entering and leaving a tunnel should be the same (when there are no other exits or parking spaces). An adversary may potentially use such information to reverse engineer the privacy protection perturbation mechanisms~\cite{rezaei19privacy,rezaei21influencers}. 
%For example, municipal agencies need to document periodical total service requests within city districts \cite{nyc2021}, while keeping confidential the exact location, time and identity of the requester. Mobility data, extracted from  phone applications or GPS devices of commute vehicles, need to deliver accurate daily or monthly traffic volumes without revealing personal trajectories \cite{sui2016characterizing,yang2019revisiting,yang2020lbsn2vec,wang2020distributed}. 
Invariants pose a new challenge to both the curators and the users of private data products, prompting its recognition as a new source of compromise to privacy that stems from external mandates.

% the output data product from the Bureau's pipeline tends to associate
%In order for the data products to satisfy invariants, the DAS employs an additional procedure,  to impose these truth constraints on the differentially private noisy measurements. 
%Unfortunately, the post-processing within the DAS introduces systematic bias into simple statistical summaries on the output data.

%A notable bias is that the output data product from the Bureau's pipeline tends to associate positive errors with larger counts and negative errors with smaller counts, when total count is held as invariant. Figure~\ref{fig:census_trend} illustrates this phenomenon using the Census Bureau's own demonstration data products (\cite{ipums2020das}, vintage 20201116), which consists of both the original values from the 2010 Census Summary File as well as their differentially private counterparts produced by the new DAS pipeline. 

%{\bf  [An important use case: Census DAS and its failures]} As a major innovation to its traditional Disclosure Avoidance System (DAS), the 2020 Decennial Census endorses differential privacy as the new standard to protect privileged information of individual respondents.





\begin{figure*}[t]
\centering
\includegraphics[width = .32\textwidth]{figs/dp_error_trend_by_county.pdf}
\includegraphics[width = .55\textwidth]{figs/sdp_error_by_county_17.pdf}
\caption{\label{fig:census_trend} Left: the Census DAS associates positive errors with larger counties and negative errors with smaller counties, when the state population is held as invariant \cite[Nov 2020 vintage demonstration files;][]{ipums2020das}. 
%For all states and  territories with more than five counties, a simple regression is performed using the log true county population as the explanatory variable and the DAS error as the response. Depicted are the least square slope estimates, out of which 37 are negative, and a further 11 are statistically significant at $\alpha = 0.01$ level (circled in red). 
Eleven out of 48 simple regressions of the county-level DAS errors against log true county populations have statistically significant negative slopes ($\alpha = 0.01$), circled in red. Right: for the counties of Illinois in increasing true population sizes, DAS errors (red squares) show a clear negative trend bias. The boxplots show errors from ten runs of our proposed method (the $(\epsilon,0)$-induced subspace differentially private projected Laplace mechanism; \Cref{cor:projected_laplace}). As  Corollary~\ref{cor:unbiasedness} shows, these errors are unbiased.}

\end{figure*}


% \begin{figure}
% \centering
% \includegraphics[width = .37\textwidth]{figs/dp_error_trend_by_county.pdf}
% \includegraphics[width = .62\textwidth]{figs/sdp_error_by_county_17.pdf}
% \vspace*{-4mm}
% \caption{\label{fig:census_trend} \small Analysis on the November 2020 vintage Census demonstration data files \cite{ipums2020das}. Left: the Census DAS associates positive errors with larger counties and negative errors with smaller counties, when the state population is held as invariant. 
% %For all states and  territories with more than five counties, a simple regression is performed using the log true county population as the explanatory variable and the DAS error as the response. Depicted are the least square slope estimates, out of which 37 are negative, and a further 11 are statistically significant at $\alpha = 0.01$ level (circled in red). 
% Eleven out of 48 simple regressions of the county-level DAS errors against log true county populations have statistically significant negative slopes ($\alpha = 0.01$), circled in red. Right: for the counties of Illinois in increasing true population sizes, DAS errors (red squares) show a clear negative trend bias. In comparison, the boxplot of errors from ten runs of our proposed methods (the  $(\epsilon,0)$-induced subspace differentially private projected Laplace mechanism defined in \Cref{cor:projected_laplace}) show no such bias. }
% \vspace*{-4mm}
% \end{figure}

%imposed by the Census Bureau's DAS as shown in the 2010 demonstration data files, vintage 2020-11-19 \cite{ipums2020das}. Both the subspace DP and DAS mechanisms preserve total state population as invariant. Due to the nature of its post-processing, however, DAS systematically imposes positive bias for smaller counties, and negative bias for larger ones, whereas the proposed mechanism maintains element-wise unbiasedness of the noisy counts.

\noindent\textbf{Our contribution}
To meet the challenge posed by invariants, we argue that the definition of differential privacy must be recapitulated to respect the given constraints. To this end, we propose the definition of \emph{subspace differential privacy}, which makes explicit the invariants imposed on the data product. Subspace differential privacy intends to honestly characterize the dependence of the privatized data product on truthful aspects of the confidential data, to ensure that any privacy guarantee attached to the data product is both mathematically rigorous and intuitively sensible. It enables the assessment of what kind of queries do, and do not, enjoy the protection of differential privacy. 

The literature has seen attempts to generalize beyond the classic notion of differential privacy. The framework of {Pufferfish} privacy~\cite{kifer2012rigorous,kifer2014pufferfish,song2017pufferfish} specifies the potential secrets, discriminative pairs, as well as the data generation model and knowledge possessed by the potential attacker. Special cases of the Pufferfish framework include {Blowfish} privacy~\cite{He2014-id} and Bayesian differential privacy~\cite{Yang2015-bc}. Related notions of correlated differential privacy \citep{zhu2014correlated} and dependent differential privacy \citep{liu2016dependence} specifically address secrets in the form of query correlations or structural dependence of the database. 

The current work differentiates itself from the existing literature in two senses. First, the theoretical focus is to provide a principled reconciliation between the hard truth constraints which the data curator must impose on the sanitized data product, and the privacy guarantee the product can enjoy. In particular, just like the classic notion of differential privacy, \emph{subspace differential privacy} does not require the specification of a data generation model nor any knowledge that the attacker might possess. Second, the practical emphasis is on the design of probabilistic mechanisms that impose deterministic truth constraints as they instill subspace differential privacy in the data product. This forgoes the need for additional post-processing, and preserves good statistical qualities of the output.

%\fang{consistency and induced privacy}
A related, but different, line of work in the literature concerns the \emph{internal} consistency of the privacy mechanism output~\cite{barak2007privacy,hay2009boosting}. For example, when we query the number of students in a school and the numbers of students in each class of the school, we may expect the outputs to be non-negative, and the sum of the (privatized) numbers of students in all classes to be equal to the (privatized) number of students in the school. These internal consistency requirements, such as non-negativity and relational constraints, are \emph{independent} of the private dataset. Therefore, they may be compatible with the classic notion of differential privacy, in which case they may be instantiated with differentially private mechanisms. However, for invariants that are nontrivial functions of the confidential data, we show in Section~\ref{sect:pre_priv} that it is impossible to have differentially private mechanisms that satisfy them. It is this kind of invariants that motivate our work in this paper.
%\jie{this two sentences are a bit confusing} \fang{rewrite it a little.  I will take another look tomorrow.}
%\robin{How about this?}
%\jie{need to add connection/comparison with our definitions/objectives}
%% \fang{Pufferfish, induced neighborhood, and linear subspace constraints}
%\robin{add more to what we want to do}
%\paragraph{Our contribution.} 

The remainder of this paper is organized as follows. Section~\ref{sec:sdp} defines \emph{subspace differential privacy} and \emph{induced subspace differential privacy}, motivated by the pair of necessary criteria that the mechanism be simultaneously provably private and invariant-respecting. Section~\ref{sec:design} outlines two general approaches, \emph{projection} and \emph{extension}, to design induced subspace differentially private mechanisms.  We apply both frameworks to produce Gaussian and Laplace mechanisms for general queries, present a correlated Gaussian mechanism that is  \emph{near-optimal} (i.e. in terms of mean squared error, with a small multiplicative factor) for linear queries, and sketch the design for a $k$-norm mechanism that would enjoy near optimality. Section~\ref{sec:discussion} discusses the statistical and implementation considerations behind the proposed mechanisms, as they enjoy transparency and statistical intelligibility that facilitate principled downstream statistical analysis. In the special case of additive spherical Gaussian mechanism, a distributional equivalence is established between the projection framework and statistical conditioning. All mechanisms can also be adapted for distributed privatization.  Section~\ref{sec:example} provides two demonstrations of the proposed induced subspace differentially private mechanisms, on the 2020 Census DAS demonstration data and spatio-temporal mobility dataset on a university campus subject to various marginal total invariants.  Section~\ref{sec:conclusion} concludes. 

%\robin{Intuitive explanation to what are we trying to do.}

%{\color{red} Question. Are we only restricted to protecting induced neighbors or can we do something greater than that?}

%\fang{Brief outline: two frameworks,  case study: Gaussian, statistical consideration, case study: Laplace and exponential}

\section{Recapitulating Privacy under Invariants}\label{sec:sdp}

%\robin{One of our revieweres did not like the word ``recapitulate''. Do we want to use something else?}\fang{I think it's fine}

In this work, we model private data as a database $\x=\left(x_{1},\dots,x_{N}\right)^{\top} \in  \mathcal{X}^N$ of $N$ rows, where each row $x_i\in \mathcal{X}$ contains data about an individual $i$, and $\mathcal{X}$ is finite with size $d$, and we set the space of all possible non-empty databases as $\mathcal{X}^*:=\cup_{N\ge 1}\mathcal{X}^N$.  
A trusted curator holds the database $\x\in \mathcal{X}^*$, and provides an interface to the database through a randomized mechanism $M:\mathcal{X}^*\to \mathcal{Y}$ where  $\mathcal{Y}\subseteq \mathbb{R}^n$ is the \emph{output space} of $M$.  We want to design good mechanisms to answer a query $A:\mathcal{X}^*\to \mathcal{Y}$ that satisfies not only certain privacy notions, but also invariant constraints as motivated in Section~\ref{sec:intro}.

We begin the discussion about mechanisms for a general query, defined by a function $A:\mathcal{X}^*\to \mathcal{Y}$, throughout the end of Section~\ref{sec:general}. In Section~\ref{sec:linear}, we consider optimal mechanisms for a \emph{linear} query $A$, with  $a:\mathcal{X}\to \mathbb{R}^n$ so that $A(\x) := \sum_{i} a(x_i)$.  Indeed, a linear query $A$ can be represented as a linear function of the \emph{histogram} of database $\x$, $\hist(\x):\mathcal{X}^*\to \mathbb{N}^{d}$ where $\hist(\x)_z := \sum_{i}\mathbf{1}[x_i = z]$ is the number of rows equal to $z\in \mathcal{X}$ in $\x\in \mathcal{X}^*$.  With this notation, given a linear query $A$, we denote $\A$ as a matrix where the $k,z$ entry is $A(z)_k$ for $k\in [n]$ and $z\in \mathcal{X}$, and the linear query on a database $\x$ can be written as matrix multiplication, 
$A(\x) = \A \cdot \hist(\x)$.
% We first define our query model and our notion of accuracy in Sect.~\ref{sect:pre_query}.  Then we introduce additional privacy or invariant constraints in Sect.~\ref{sect:pre_priv}.



\subsection{Privacy Guarantees and Invariants}\label{sect:pre_priv}
% Besides providing accurate output answering query $A$, our mechanism $M$ needs to protect individuals' privacy.  Thus, instead of all functions from $\mathcal{X}^*$ to $\mathbb{R}^n$, our mechanism $M$ can be only in a restricted set $\mathscr{M}$.

The notion of differential privacy ensures that no individual's data has much effect on the output of the mechanism $M$.  That is, if we consider any two neighboring databases $\x$ and $\x'$ of size $N$ that differ on one row (there exists $i$ such that $x_i \neq x_i'$ and  $x_j = x_j'$ for all $j\neq i$.) the output distribution of mechanism $M$ on $\x$ should be similar to that of $M$ on $\x'$.  Formally:
\begin{definition}[Bounded differential privacy~\cite{dwork2006calibrating}]\label{def:dp}
%Let $A:\mathcal{X}^* \to\mathbb{R}^{n}$ be a deterministic query function. 
Let $(\mathcal{Y}, \mathcal{F})$ be a measurable space and $\epsilon, \delta\ge0$. We say that a random mechanism $M: \mathcal{X}^*\to\mathcal{Y}$ is \emph{$\left(\epsilon,\delta\right)$-differentially private} if for all neighboring databases $\x\sim \x'$ and all measurable set $S\in\mathcal{F}$, 
$\Pr\left[ M\left(\x\right)\in S\right]\le e^\epsilon\cdot \Pr\left[M\left(\x'\right)\in S\right]+\delta$.
\end{definition}

From the data curator's perpective, in addition to privacy concerns, there often exists external constraints that the privatized output $M$ must meet. 
%For instance, we want to publish the histogram but also ensure the the number of agents is invariant (Example~\ref{ex:hist}). 
These constraints can often be represented as a function of $M(\x)$ that agrees with what's calculated based on the confidential $A(\x)$. In this work, we focus on the class of invariants that can be written in the form of a system of linear equations. 
\begin{definition}[Invariants - linear equality]\label{def:invariant}
Given a query $A:\mathcal{X}^*\to \mathbb{R}^n$, and $C\in \mathbb{R}^{n_c\times n}$ be a $n_c\times n$ matrix with rank $n_c<n$.\footnote{We can always find a $C'$ consists of a subset of independent rows of $C$ which has same row rank as $C$'s,  and we can translate between these two through a linear transformation.} A (random) mechanism $M:\mathcal{X}^*\to \mathcal{Y}\subseteq \mathbb{R}^n$ satisfies the \emph{linear equality invariant $C$ with query $A$}, if for all $\x$,
$CM\left({\bf x}\right) =CA(\x)$ with probability one over the randomness of $M$. 
\end{definition}
Given a linear equality invariant $C$, let $\mathcal{N} :=\{v\in \mathbb{R}^n:Cv = 0\}$ be the \emph{null space} of $C$, and $\mathcal{R} := \mathcal{N}^\perp\subseteq\mathbb{R}^n$ be the \emph{row space} of $C$.  Additionally, we set $\Pi_\mathcal{N}$ be the orthogonal projection matrix for null space $\mathcal{N}$, $Q_\mathcal{N}$ be a collection of orthonormal basis of $\mathcal{N}$, and $A_\mathcal{N}:= Q_\mathcal{N}^\top A$ be the query function $A$ projected into $\mathcal{N}$ with basis $Q_\mathcal{N}$.  We use subscript $\mathcal{R}$ in the similar manner.  

Linear equality invariants are a natural family of invariants. Here are two examples. 
\begin{example}\label{ex:hist}
Let $\x\in \mathcal{X}^N$ be a database with $|\mathcal{X}| = d$, $A = \hist$ be the histogram query, and $C = \mathbf{1}^\top = (1,\dots,1)\in \mathbb{R}^{1\times d}$ all one vector with length $d$. 
This linear equality invariant requires the curator to accurately report the total number of individuals without error, because $CM(\x) = \mathbf{1}^\top \hist(\x) = N$.
\end{example}

\begin{example}\label{ex:even}
Consider $\mathcal{X} = \{1,2,3,4\}$, $A = \hist: \mathcal{X}^*\to \mathbb{R}^4$ and $C = (1, 0, 1, 0)$.  The linear equality invariant ensures the number of individual with odd feature is exact.
\end{example}

The invariants discussed in the Census DAS application, such as state-level population and block-level housing units and group quarter facilities, can be formulated as linear equality invariants.
%{\color{blue} For example, the state population total, etc can be written this way...} \jie{I want to connect back to the applications in the introduction}

%\robin{Beginning from here we lay out the core of subspace differential privacy, Do we want to start a new subsection? }

\subsection{Subspace and Induced Subspace Differential Privacy}


% \fang{discussed in?}
% 	\item maintain the practicality of implementation as well as the statistical intelligibility of the output.
% \subsection{Subspace Differential Privacy}
%\robin{this can be shortened}

The mechanism we seek must meet two necessary criteria: \emph{provably private} and \emph{invariant-respecting}. That is, the mechanism should privatize the confidential query with mathematically provable guarantees, while at the same time the query output should conform to the invariants that a data curator chooses to impose. The two criteria culminate in the \emph{\goodprivacynoun} (\Cref{def:isubdp}) which enjoys additional desirable properties, such as the practicalities of design and statistical intelligibility, which will be discussed from \cref{sec:design} and on.

To motivate the construction,  note that the classic definition of differential privacy and invariant constraints are not compatible by design.  For instance, in Example~\ref{ex:even} if a mechanism $M$ respects the invariant constraint~\Cref{def:invariant}, the probability ratio of event $S = \{(y_1, y_2, y_3, y_4): y_1+y_3 = 1\}\subset \mathbb{R}^4$ on  neighboring databases $\x = (1,2,4)$ and  $\x' = (4,2,4)$ is unbounded, $\frac{\Pr[M(\x)\in S]}{\Pr[M(\x')\in S]}=\infty$,
because $\Pr[M(\x)\in S] = \Pr[CM(\x) = C\hist(\x)] = 1$ but $\Pr[M(\x')\in S] = \Pr[CM(\x') \neq C\hist(\x')] = 0$.  Thus $M$ violates $(\epsilon, \delta)$-differential privacy for any $\epsilon>0$ and $\delta<1$.  

Therefore, we need a new notion of differential privacy to discuss the privacy protection in the presence of mandated invariants. Below we attempt to do so by recapitulating the definition of  $\left(\epsilon,\delta\right)$-differential privacy, to acknowledge the fact that if a hard linear constraint is imposed on the privacy mechanism, we can no longer offer differential privacy guarantee in the full $n$-dimensional space that is the image of $A$, but rather only within certain linear subspaces.


\begin{definition}[Subspace differential privacy]\label{def:subdp}
%Let $A:\mathcal{X}^*\to\mathbb{R}^{n}$ be a query function operating on database ${\bf x}\in\mathcal{X}^*$. 
Let $\mathcal{V}$ be a linear subspace of $\mathbb{R}^{n}$, and $\Pi_{\mathcal{V}}$ the projection matrix onto $\mathcal{V}$. Given $\epsilon, \delta\ge 0$, a random mechanism $M:\mathcal{X}^*\to\mathbb{R}^{n}$ is \emph{$\mathcal{V}$-subspace $\left(\epsilon,\delta\right)$-differentially private} if for all neighboring databases ${\bf x}\sim {\bf x}'$ and { every Borel subset $S\subseteq \mathcal{V}$}, %\fang{why Borel measurable instead of Lebesgue?}\robin{This is because $S$ is in the range of a random variable. It needs to be a Borel subset of $\mathcal{V}$ in order for $\Pr$ to spit out a number}
\begin{equation}
\Pr\left[ \Pi_{\mathcal{V}} M\left({\bf x}\right)\in S\right]\le e^\epsilon\Pr\left[\Pi_{\mathcal{V}}M\left({\bf x}'\right)\in S\right]+\delta.
\end{equation}
\end{definition}
%\robin{REFER TO APPENDIX - NESTED PROPERTY, and motivate this proposition} 

%It establishes that subspace differential privacy is more general, hence logically weaker, than differential privacy. 

%\fang{need to justify $\mathcal{N}$-subspace differentially private}.
%With invariants and subspace differential privacy defined, 

We are ready to formalize the notion of a provably private and invariant-respecting private mechanism, one that meets both the criteria laid out at the beginning of this subsection.  
\begin{definition}[Induced subspace differential privacy]\label{def:isubdp}
Given $\epsilon, \delta\ge 0$, a query $A:\mathcal{X}^*\to \mathbb{R}^n$ and a linear equality invariant $C:\mathbb{R}^n\to \mathbb{R}^{n_c}$ with null space $\mathcal{N}$, a mechanism $M:\mathcal{X}^*\to \mathbb{R}^n$ is \emph{$(\epsilon, \delta)$-\goodprivacy for query $A$ and an invariant $C$} if 
%\begin{enumerate}\denselist
%\item 
1) $M$  is $\mathcal{N}$-subspace $(\epsilon, \delta)$-differentially private (\Cref{def:subdp}), and 
%\item 
2) $M$ satisfies the linear equality invariant $C$ (\Cref{def:invariant}).
%\end{enumerate}
$\mathcal{M}$ may be referred to simply as \emph{\goodprivacy}, whenever the context is clear about (or does not require the specification of) $\epsilon, \delta$ and $C$.
\end{definition}
An \goodprivacy mechanism delivers query outputs that meet the curator's invariant specification ($C$) with probability one. It is provably differentially private for all queries and their components that are orthogonal to the invariants, and is silent on privacy properties for those that are linearly dependent on the invariants. 

\subsection{Properties of Subspace Differential Privacy} 

%\jie{I collected properties of subspace DP here. please check}
Now we discuss several properties of subspace differential privacy. First, we show a ``nestedness'' property:  a $\mathcal{V}_1$-subspace differentially private mechanism is also $\mathcal{V}_2$-subspace differentially private for all $\mathcal{V}_1\supseteq \mathcal{V}_2$.

\begin{proposition}\label{prop:nested}
Let ${\mathcal{V}}_2 \subseteq {\mathcal{V}_1}$ be nested linear subspaces of respective dimensions $d_2 \le d_1$. If a mechanism $M$ is ${\mathcal{V}_1}$-subspace $\left(\epsilon,\delta\right)$-differentially private, it is also ${\mathcal{V}}_2$-subspace $\left(\epsilon,\delta\right)$-differentially private.
\end{proposition}

The main idea is that because $\mathcal{V}_2\subseteq \mathcal{V}_1$ are both linear spaces, for any measurable $S$, we can always find another measurable set $S'$ such that $\Pi_{\mathcal{V}_2}^{-1}(S) = \Pi_{\mathcal{V}_1}^{-1} (S')$.  Thus $\mathcal{V}_1$-subspace differential privacy implies $\mathcal{V}_2$-subspace differential privacy.  We include the proof to the appendix.



\Cref{prop:nested} implies that a differentially private mechanism is subspace differential private, as shown in \Cref{prop:unconstrained}.  Thus, we can call an  $\left(\epsilon,\delta\right)$-differentially private mechanism the $\mathbb{R}^n$-subspace $\left(\epsilon,\delta\right)$-differentially private mechanism.   
\begin{corollary}[label = prop:unconstrained]
If $M:\mathcal{X}^*\to \mathbb{R}^n$ is a $\left(\epsilon,\delta\right)$-differentially private mechanism, it is $\mathcal{V}$-subspace $\left(\epsilon,\delta\right)$-differentially private for any linear subspace $\mathcal{V} \subseteq \mathbb{R}^n$.
\end{corollary}



%\fang{new}
Induced subspace differential privacy inherits the composition property from differential privacy in the following sense (with proof in Appendix~\ref{app:subspace}).
\begin{proposition}[name=Composition, label = prop:composition, restate=Composition]
Given $\epsilon_1\ge 0$ and $\epsilon_2\ge 0$, 
% query functions $A_1:\mathcal{X}\to \mathcal{Y}_1$ and $A_2:\mathcal{X}\to \mathcal{Y}_2$, and linear invariant $C_1: \mathcal{Y}_1\to \mathcal{Z}_1$ and $C_2: \mathcal{Y}_2\to \mathcal{Z}_2$, 
if $M_1$ is induced subspace $(\epsilon_1,0)$-differentially private for query $A_1$ and linear invariant $C_1$ and $M_2$ is induced subspace $(\epsilon_2,0)$-differentially private for query $A_2$ and linear invariant $C_2$, the composed mechanism $(M_1, M_2)$ is induced subspace $(\epsilon_1+\epsilon_2,0)$-differentially private for query $A_{1,2} := (A_1, A_2)$ and linear invariant $C_{1,2} := (C_1, C_2)$. 
\end{proposition} 


The above is a preliminary answer to the composition property of subspace differential privacy. %{\color{blue} 
However, when $C_1$ and $C_2$ are different, the composition of invariant constraints may reveal additional information about the underlying confidential data. In general, the composition of logically independent  and informative invariants is not unlike a database linkage attack. 
For instance, $A_1 = A_2$ is a two-way contingent table that reports the counts of individuals with ages and zip code, the invariant $C_1$ ensures the accurate marginal counts of individuals within each age bracket, and $C_2$ ensures the accurate count of individuals within each zip code.  The composition of these two invariant constraints may allow an adversary to infer each individual's information.  


%\robin{Can we make this a bit more formal, e.g. as a proposition?}\fang{I am good with the current discussion.  Linear post processing is too restrictive and formally factoring the function is too artificial.} 
The subspace differential privacy is naturally immune to any post-processing mapping which only acts on the subspace $\mathcal{N}$. However, it is not readily clear how to define post-processing under mandated invariant constraints.  Specifically, if a mechanism satisfies a nontrivial invariant constraint $C$ with row space $\mathcal{R}$ and null space $\mathcal{N}$, we can apply a post-processing mapping that outputs the invariant component in $\mathcal{R}$ -- here the output is revealed precisely. Unfortunately, such will be true for any invariant-respecting privatized product, regardless of what notion of privacy is attached to it. 



%We present the proof and discussion of post-processing in Appendix~\ref{app:subspace}.

%\jie{Convexity}\fang{added here}
Finally, we note that if we consider a mixture of two $\mathcal{V}$-subspace differentially privacy mechanisms the resulting mechanism is also $\mathcal{V}$-subspace differentially private.  This property is known as the privacy axiom of choice~\cite{kifer2010towards}.



\section{Mechanism Design}\label{sec:design}

This section introduces two frameworks for designing \goodprivacy mechanisms with linear equality invariant $C$. 
The data curator would invoke the \emph{projection} framework if seeking to impose invariants onto an \emph{existing} differentially private mechanism, and the \emph{extension} framework if augmenting a smaller private query in a manner compatible with the invariants. Both frameworks are applied to revise existing differentially private mechanisms in \Cref{sec:general}, notably the Gaussian and the Laplace mechanisms, for general queries. For linear queries, \Cref{sec:linear} presents a near optimal correlated Gaussian mechanism, and sketches the design of a near optimal $k$-norm mechanism.

 
\subsection{The Projection Framework}\label{sec:projection}

Suppose the data curator already employs a differentially private mechanism $M$ to answer a general query $A$, and would like to impose a linear equality invariant $C$ on the query output. The projection framework, outlined in~\Cref{thm:projection}, can transform the existing mechanism $M$ to \goodprivacy for $A$ and $C$, with little overhead on the curator's part. 

\begin{theorem}[Projection framework]\label{thm:projection}
Given $\epsilon, \delta\ge 0$, a general query $A:\mathcal{X}^*\to \mathbb{R}^n$, and a linear equality invariant $C$ with null space $\mathcal{N}$, if $M:\mathcal{X}^*\to \mathbb{R}^n$ is $(\epsilon, \delta)$-differentially private, then $\mathcal{M}(\x):=A(\x)+\Pi_\mathcal{N}(M(\x)-A(\x))$, for all $\x\in \mathcal{X}^*$ is $(\epsilon, \delta)$-\goodprivacy for query $A$ and invariant $C$.
\end{theorem}
Informally, we conduct projection on a differentially private mechanism in order to 1) remove the noise in the row space of $C$ to respect the invariant constraint $C$; and 2) preserve noise in the null space $\mathcal{N}$ and satisfy $\mathcal{N}$-subspace differential privacy. 
%\robin{incomplete sentence?}

\begin{proof}[Proof of Theorem~\ref{thm:projection}]
Because for all $\x\in \mathcal{X}^*$, $C\mathcal{M}(\x)=C A(\x)+C\Pi_{\mathcal{N}}(M(\x)-A(\x)) = CA(\x)$, 
$\mathcal{M}$ satisfies the invariant $C$.
Since $M$ is $\mathcal{N}$-subspace $(\epsilon, \delta)$-differentially private by \Cref{prop:unconstrained}, and  $\Pi_{\mathcal{N}}\mathcal{M}(\x)$ equals $\Pi_{\mathcal{N}}M\left(\x\right)$ in distribution, $\mathcal{M}$ is also ${\mathcal{N}}$-subspace differentially private.
\end{proof}

%\paragraph{Additive mechanisms} 
%\robin{I removed the paragraph title, since the word "additive" is already italicized so this may read okay.} 

The projection framework in \Cref{thm:projection} is particularly useful for revising \emph{additive} mechanisms, having the form
\begin{equation}\label{eq:additive}
M(\x) = A(\x)+\mathbf{e},	
\end{equation}
where ${\bf e}$ is a noise component independent of $A(\x)$. Examples of additive mechanisms include the classic Laplace and Gaussian mechanisms~\citep{dwork2006calibrating}, $t$-\citep{nissim2007smooth}, double Geometric \citep{fioretto2019differential}, and $k$-norm mechanisms~\citep{hardt2010geometry,bhaskara2012unconditional}. In contrast, the Exponential mechanism~\citep{mcsherry2007mechanism} is in general not additive because the sampling process depends on the utility function non-additively.  

% he $k$-norm mechanism and correlated Gaussian mechanism~\cite{nikolov2013geometry} induce correlations among dimensions of the privatization noise.  By Theorem~\ref{thm:projection}, we have the following corollary for additive privatization mechanisms.

When the existing differentially private mechanism $M$ is additive, the projection construction of an \goodprivacy mechanism based on $M$ can be simplified, by first sampling the noise $\mathbf{e}$, and outputting the query value $A(\x)$ with the projected noise added to it.
\begin{corollary}\label{cor:projection}
If the mechanism $M$ in Theorem~\ref{thm:projection} is furthermore additive, i.e. of the form~\eqref{eq:additive}, the modified mechanism,
$\mathcal{M}(\x):=A(\x)+\Pi_{\mathcal{N}}\mathbf{e}$,
% \begin{equation*}
% \mathcal{M}(\x):=A(\x)+\Pi_{\mathcal{N}}\mathbf{e} %\label{eq:additive-projection}
% \end{equation*}
is $(\epsilon, \delta)$-\goodprivacy for query $A$ and invariant $C$. 
\end{corollary}

% As a special case, if $M$ is the widely employed spherical Gaussian mechanism (to be defined in~\Cref{lem:gaussian}), the constructed $\mathcal{M}$ further enjoys an equivalence between the projection to, and the probabilistic conditioning on the invariant margin. This greatly facilitates principled downstream statistical analysis. We defer the discussion on this matter to \Cref{sec:discussion}. \jie{This paragraph is a bit early? maybe we should move it to section 3.3?}
%\robin{Say that 3.2 and 3.3 will use this. }

\Cref{cor:projection} will be useful for the derivation of the projection mechanisms, as well as the various statistical properties of additive mechanisms (including the crucial \emph{unbiasedness} property), to be discussed in the ensuing sections.  

\subsection{The Extension Framework}\label{sec:extension}

The projection framework in Section~\ref{sec:projection} transforms an existing differentially private mechanism to one that is subspace differentially private and respects the invariant $C$. The extension framework, on the other hand, enables the design of an \goodprivacy mechanism without a full mechanism in place yet. \Cref{thm:connect} discusses how to extend a differential private mechanism with image contained in $\mathcal{N}$ to an \goodprivacy mechanism.  Moreover, the converse also holds--- any \goodprivacy mechanism can be written as a differential private mechanism with a translation. Thus, the extension framework provides the optimal trade-off between privacy and accuracy, as \Cref{cor:err_constrain2dp} will show.  We defer the proof to supplementary material.


\begin{theorem}[name = Extension framework,label = thm:connect,restate = connect]
Given $\epsilon, \delta\ge 0$, a general query $A:\mathcal{X}^*\to \mathbb{R}^n$, and a  linear equality invariant $C$ with null space $\mathcal{N}$ and row space $\mathcal{R}$, $\mathcal{M}$ is $(\epsilon, \delta)$-\goodprivacy for query $A$ and invariant $C$, if and only if 
$\mathcal{M}(\mathbf{x}):=\hat{M}(\mathbf{x})+\Pi_{\mathcal{R}} A(\x)$
where $\hat{M}$ is $(\epsilon, \delta)$-differentially private and its image is contained in $\mathcal{N}\subseteq \mathbb{R}^n$.
\end{theorem}




\subsection{Induced Subspace Differentially Private Mechanisms for General Queries}\label{sec:general}

We now describe the use of the above two frameworks to construct \goodprivacy mechanisms.  We first introduce \goodprivacy mechanisms with Gaussian noises, then the pure (i.e. $\delta = 0$) versions with Laplace noises.
All mechanisms discussed in this section are additive mechanisms, having a general functional form as \eqref{eq:additive}.


Let the \emph{$\ell_{p}$ sensitivity} of the query function $A:\mathcal{X}^*\to \mathbb{R}^n$ be
$\Delta_{p}(A) = \sup_{{\bf x}\sim {\bf x}'}\left\Vert A({\bf x}) - A({\bf x}') \right\Vert _{p}$, which  measures how much a single individual's data can change the output of the query $A$. We measure the performance of a mechanism $M$ in terms of the expected squared error.
Given any query function $A: \mathcal{X}^* \to \mathbb{R}^n$, the worst-case expected squared error of a mechanism $M$ for $A$ is defined as $\err_M(A):=\sup_{\x\in \mathcal{X}^*}\E\left[\|M(\x)-A(\x)\|^2_2\right]$.
%, and we will call a mechanism $M$ is additive for a query $A$ with noise $\mathbf{e}$ if $M(\x) = A(\x)+\mathbf{e}$ for all $\x$. 

\noindent\textbf{Gaussian mechanisms}
%\paragraph{Gaussian mechanisms}
Recall the standard Gaussian mechanism, which adds a spherical noise to the output that depends on the $\ell_2$ sensitivity of $A$.   By an abuse of notation, the superscript $n$ over a probability distribution denotes the $n$-dimensional product distribution with the said marginal. 

\begin{lemma}[name=Gaussian mechanism~\cite{dwork2006our}, label=lem:gaussian]
For all $\epsilon, \delta>0$, and general query $A:\mathcal{X}^*\to \mathbb{R}^n$, let $c_{\epsilon, \delta}:= \epsilon^{-1}(1+\sqrt{1+\ln(1/\delta)})$.  
Then an additive mechanism for $A$ with noise $\mathbf{e}_{G}(A, \epsilon, \delta) \overset{d}{=} N(0;  \Delta_2(A)c_{\epsilon, \delta})^n$ where $N(0; \sigma)$ is the unbiased Gaussian distribution with variance $\sigma^2$ $(\epsilon, \delta)$-differentially private.
\end{lemma}

Given $\epsilon, \delta>0$, a general query $A:\mathcal{X}^*\to \mathbb{R}^n$, and linear equality invariant $C\in \mathbb{R}^{n_c\times n}$, by projection (\Cref{thm:projection}) and extension (\Cref{thm:connect}), we can derive two \goodprivacy Gaussian mechanisms.  
The proofs of Corollaries~\ref{cor:projected_gaussian} and~\ref{cor:extended_gaussian} are both given in Appendix~\ref{app:general}.  

% Instead of adding the spherical noise, by \Cref{thm:projection} we can add a projected the noise in the null space $\mathcal{N}$ for the linear equality invariant, and get a Gaussian \goodprivacy mechanism.  Because our noise term is spherically symmetric, the error bound is controlled by the $\ell_2$ sensitivity of $A$ and the dimension of null space, $n-n_c$.

\begin{corollary}[name=Projected Gaussian mechanism, label=cor:projected_gaussian]
An additive mechanism $\mathcal{M}_{PG}$ for $A$ with noise $\Pi_\mathcal{N}\mathbf{e}_{G}(A, \epsilon, \delta)$ where $\mathbf{e}_{G}$ is defined in \Cref{lem:gaussian} is $(\epsilon, \delta)$-\goodprivacy for query $A$ and invariant $C$. 
Moreover, 
$\err_{\mathcal{M}_{PG}}(A) = (n-n_c)c_{\epsilon, \delta}^2\Delta_2(A)^2$.
\end{corollary}

%\fang{proof of the error in the supplementary material}
%\robin{Say a few words here about how \Cref{cor:projected_gaussian} is equivalent to \Cref{cor:projection}?}

To apply the extension framework of~\Cref{thm:connect},  one complication is how to design a differentially private mechanism with image in $\mathcal{N}$.  To handle this, we first project the query $A$ to the null space $\mathcal{N}$ and have a new query $A_\mathcal{N} = Q_\mathcal{N}^\top A: \mathcal{X}^*\to \mathbb{R}^{n-n_c}$. Then, compute the sensitivity of $A_\mathcal{N}$, $\Delta_2(A_\mathcal{N})$, and sample $\mathbf{e}_\mathcal{N}$ which consists of $n-n_c$ iid Gaussian noise with variance $(c_{\epsilon, \delta}\Delta_2(A_\mathcal{N}))^2$.  Finally, convert the noise to the original space $\mathbb{R}^n$ and add the true query $A(\x)$.  We define the mechanism formally below.
\begin{algorithm}[htb]
\caption{Gaussian \goodprivacy mechanism through extension}
\label{alg:gaussian_extended}
\textbf{Input}: a database $\x$, a query $A:\mathcal{X}^*\to \mathbb{R}^n$, linear equality invariant $C\in \mathbb{R}^{n_c\times n}$ with rank $n_c$, $\epsilon\in (0,1)$, and $\delta\in (0,1)$.
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Compute $Q_\mathcal{N}\in \mathbb{R}^{n\times n-n_c}$ an collection of an orthonormal basis of $\mathcal{N}$, and $A_\mathcal{N}:= Q^\top_\mathcal{N}A$.
\STATE Let $c_{\epsilon, \delta} = \epsilon^{-1}(1+\sqrt{1+\ln(1/\delta)})$, and sample $\mathbf{e}_\mathcal{N}\overset{d}{=} N\left(0;c_{\epsilon, \delta}\Delta_2(A_\mathcal{N})\right)^{n-n_c}.$
\STATE \textbf{return} $A(\x)+Q_\mathcal{N} \mathbf{e}_\mathcal{N}$.
\end{algorithmic}
\end{algorithm}



\begin{corollary}[name=Extended Gaussian mechanism, label=cor:extended_gaussian]
An additive mechanism $\mathcal{M}_{EG}$ for $A$ with noise $\mathbf{e}_{EG}(A, \epsilon, \delta) = Q_\mathcal{N}e_\mathcal{N}$ where $e_\mathcal{N}\overset{d}{=} N\left(0;c_{\epsilon, \delta}\Delta_2(Q_\mathcal{N}^\top A)\right)^{n-n_c}$  is $(\epsilon, \delta)$-\goodprivacy for query $A$ and invariant $C$. 
Moreover, 
$\err_{\mathcal{M}_{EG}}(A) = (n-n_c)c_{\epsilon, \delta}^2\Delta_2(Q_\mathcal{N}^\top A)^2$.
\end{corollary}


Since $Q_\mathcal{N}$ consists of orthonormal columns, the $\ell_2$ sensitivity of $Q_\mathcal{N}^\top A$ is less than or equal to the sensitivity of the original query $A$, and the error in \Cref{cor:extended_gaussian} is no more than the error in \Cref{cor:projected_gaussian}.




\noindent\textbf{Laplace mechanisms}
Similarly, the standard Laplace mechanism adds independent product Laplace noise to the output that depends on the $\ell_1$ sensitivity of $A$. In what follows, $\Lap(b)$ denotes the univariate Laplace distribution with scale $b>0$, with density function $\frac{1}{2b}\exp\left(-\frac{|x|}{b}\right)$.
\begin{lemma}[name=Laplace mechanism~\citep{dwork2006calibrating}, label=lem:laplace]
Given $\epsilon>0$, and a query $A:\mathcal{X}^*\to \mathbb{R}^n$, an additive mechanism for $A$ with noise $\mathbf{e}_L(A, \epsilon)\overset{d}{=} \Lap(  \Delta_1(A)/\epsilon)^n$ is $(\epsilon, 0)$-differentially private.
\end{lemma}
 
% By our frameworks (\Cref{thm:projection,thm:connect}), we have two Laplace \goodprivacy mechanisms
% \begin{enumerate}
%     \item For the projection framework on general query $A$, we can modify Algorithm~\ref{alg:gaussian_projected}: instead of adding Gaussian noise, We add a Laplace noise with scale $\Delta_1(A)/\epsilon$ where $\Delta_1(A):=\sup_{\x,\x'\in \mathcal{X}^*:\x\sim\x'}\|A(\x)-A(\x')\|_1$.  
%     \item Similarly, for the extension framework, we can modify Algorithm~\ref{alg:gaussian_extended}, and add a Laplace noise with scale $\Delta_1(A_\mathcal{N})/\epsilon$.
% \end{enumerate}

Given $\epsilon>0$, a query $A:\mathcal{X}^*\to \mathbb{R}^n$, and a linear equality invariant $C\in \mathbb{R}^{n_c\times n}$, we have the following two \goodprivacy Laplace mechanisms.
\begin{corollary}[name=Projected Laplace mechanism, label=cor:projected_laplace]
The additive mechanism for $A$ with noise $\Pi_\mathcal{N}\mathbf{e}_{L}$ where $\mathbf{e}_{L}$ is defined in \Cref{lem:laplace} is $(\epsilon, 0)$-\goodprivacy for query $A$ and invariant $C$. 
\end{corollary}


\begin{corollary}[name=Extended Laplace mechanism, label=cor:extended_laplace]
An additive mechanism $\mathcal{M}_{LE}$ for $A$ with noise $\mathbf{e}_{EL}(A, \epsilon) = A(\x)+Q_\mathcal{N}w_\mathcal{N}$ where $w_\mathcal{N}\overset{d}{=} \Lap\left(\Delta_1(Q_\mathcal{N}^\top A))/\epsilon\right)^{n-n_c}$ is $(\epsilon, 0)$-\goodprivacy for query $A$ and invariant $C$. 
\end{corollary}

We have thus far discussed four mechanisms, respectively derived using the projection and extension frameworks, and employing Gaussian and Laplace errors. In practice, a data curator would choose either projected mechanisms if seeking to impose invariants on an existing differentially private mechanism, and either extension mechanisms if augmenting a smaller private query while staying compatible with the invariants. The curator would prefer the Laplace mechanisms over the Gaussian ones if a pure (i.e. $\delta = 0$) subspace differential privacy guarantee is sought, although at the expense of heavier-tailed noises which may be undesirable for utility purposes. In what follows, we discuss mechanism options for the curator, if utility considerations are the most salient.
 

% \robin{A comment on practical recommendations: which one to pick for the practitioner? Also, discuss the error size in the projection mechanisms - even though they look like they're bigger but it's because they both started with fully DP mechanism can be conservative.}
% \fang{practical consideration: pure or approximate \goodprivacy, statistical meaning(conditional, projection etc), and error minimization vs overhead on existing mechanisms}



\subsection{Optimal Induced Subspace Differentially Private Mechanisms for Linear Queries}\label{sec:linear}


%\fang{I rewrite most of this section}\robin{READ this section and turn off the comments}
%\robin{For paragraph below and Corollary 17, the word "optimal" does not have "near" in front of it. Is this fine?}\fang{In \Cref{thm:sdp_corr_gaussian} I only use the first part, but not the furthermore part.  Maybe we can remove it?}



% Given a family of mechanisms $\mathscr{M}\subseteq \{M:\mathcal{X}^*\to \mathbb{R}^n\}$, the optimal error achievable by any $M\in \mathscr{M}$ for query $A$ is $
    % \opt_{\mathscr{M}}(A):=\inf_{M\in \mathscr{M}}\err_M(A)$.
    
As a consequence of \Cref{thm:connect}, \Cref{cor:err_constrain2dp} translates optimal accuracy enjoyed by a differentially private mechanism to optimal accuracy by an \goodprivacy mechanism.  Let $\opt_{\epsilon, \delta}(A)$ be the optimal error achievable by any $(\epsilon, \delta)$-differentially private mechanism, and $\opt_{\epsilon, \delta}^C(A)$ be the optimal error by any $(\epsilon, \delta)$-\goodprivacy mechanism 
for query $A$ and invariant $C$. 


\begin{corollary}\label{cor:err_constrain2dp}  For all $\epsilon, \delta\ge 0$, general query $A:\mathcal{X}^*\to \mathbb{R}^n$, and linear equality invariant $C$, 
$\opt_{\epsilon, \delta}^C(A) = \opt_{\epsilon, \delta}(\Pi_{\mathcal{N}}A)$.  
% Furthermore, if $\hat{M}$ is an optimal $(\epsilon, \delta)$-differentially private mechanism for query $\Pi_\mathcal{N}A$, $\mathcal{M}:=\hat{M}+\Pi_\mathcal{R}A$ is an optimal $(\epsilon, \delta)$-\goodprivacy mechanism for $A$ and $C$.
\end{corollary}
We defer the proof to Appendix~\ref{app:optimal}.  Informally, for any differentially private mechanism we use the extension framework in \Cref{thm:connect} to construct an \goodprivacy mechanism.  Because our proof is constructive, we can translate existing near optimal differentially private mechanisms to \goodprivacy ones.  

We demonstrate this translation with a near-optimal (i.e. mean squared error with a small multiplicative factor) correlated Gaussian mechanism for linear queries from  \citet{nikolov2013geometry}.
Specifically, first design a differential private mechanism $\hat{M}$ for $A_\mathcal{N}:=Q_\mathcal{N}^\top A$, and extend it to a subspace differentially private mechanism by Theorem~\ref{thm:connect}. Because the mean squared error is invariant under rotation, $\err_{\hat{M}}(\Pi_\mathcal{N}A) = \err_{\hat{M}}(A_\mathcal{N})$.  Therefore, if $\hat{M}$ is the near optimal correlated Gaussian noise mechanism for $A_\mathcal{N}$, the resulting \goodprivacy mechanism  is also near optimal by \Cref{cor:err_constrain2dp}.  Details of this mechanism is spelled out in \Cref{alg:subspace_gaussian} which we, together with the proof for \Cref{thm:sdp_corr_gaussian} below, defer to Appendix~\ref{app:optimal}.

\begin{theorem}\label{thm:sdp_corr_gaussian}
Given $\epsilon, \delta>0$, a linear query $A: \mathbb{R}^d\to \mathbb{R}^n$, and a linear equality invariant $C\in \mathbb{R}^{n_c\times n}$, \Cref{alg:subspace_gaussian} is an efficient $(\epsilon, \delta)$-\goodprivacy mechanism such that for all small enough $\epsilon$ and all $\delta$ small enough with respect to $\epsilon$ satisfies 
$$err_{\mathcal{M}}(A) = O(\log^2(n-n_c)\log 1/\delta)\opt_{\epsilon, \delta}^{C}(A).$$
\end{theorem}

We may use the same idea to convert an $k$-norm mechanism~\citep{hardt2010geometry,bhaskara2012unconditional} to an $(\epsilon, 0)$-\goodprivacy one.  \citet{bhaskara2012unconditional} proposed an $(\epsilon, 0)$-differentially private $k$-norm mechanism whose approximation ratio of mean squared error is $O((\log n)^2)$ for any linear query with image in $\mathbb{R}^n$.  We can run the $k$-norm mechanism on query $A_\mathcal{N}$ whose mean squared error is $O((\log (n-n_c))^2)\opt_{\epsilon,0}(A_\mathcal{N})$.  Then, by \Cref{cor:err_constrain2dp}, the output can be converted to an $(\epsilon, 0)$-\goodprivacy mechanism, with an approximation ratio $O((\log n-n_c)^2)$.
%\robin{Is this the K-norm? say a bit more here}



% \subsection{Laplace and Exponential Induced Subspace Differentially Private Mechanism}

% Besides Gaussian mechanism in Sect.~\ref{sec:gaussian}, we can adapt our frameworks in Sect.~\ref{sec:frameworks} to other existing differentially private mechanisms.  First, we can use Laplace mechanism \fang{reference} to  derive $(\epsilon,0)$-\goodprivacy mechanisms.  Then, we discuss  

% \begin{definition}[Laplace distribution] The Laplace distribution $X$ with scale $b>0$ is the distribution with probability density function: $f(x) = \frac{1}{2b}\exp\left(-\frac{|x|}{b}\right)$.
% \end{definition}

% \fang{move the following to the appendix?}


% \begin{proof}
% We consider the ratio of probability that an outcome of the exponential mechanism $y$ on two neighboring databases $\x\sim \x'$.
% \begin{align*}
%     \frac{\Pr[\mathcal{M}_E(\x) = y]}{\Pr[\mathcal{M}_E(\x') = y]} =& \frac{\exp\left(\frac{\epsilon u(\x, y)}{2\Delta(u)}\right)}{\exp\left(\frac{\epsilon u(\x', y)}{2\Delta(u)}\right)}\cdot \frac{\sum_z\exp\left(\frac{\epsilon u(\x', z)}{2\Delta(u)}\right)}{\sum_z\exp\left(\frac{\epsilon u(\x, z)}{2\Delta(u)}\right)}\\
%     =& \exp\left(\frac{\epsilon (u(\x, y)-u(\x', y))}{2\Delta(u)}\right)\cdot \frac{\sum_z\exp\left(\frac{\epsilon u(\x', z)}{2\Delta(u)}\right)}{\sum_z\exp\left(\frac{\epsilon u(\x, z)}{2\Delta(u)}\right)}\\
%     \le& \exp\left(\frac{\epsilon }{2}\right)\cdot \exp\left(\frac{\epsilon }{2}\right) \frac{\sum_z\exp\left(\frac{\epsilon u(\x, z)}{2\Delta(u)}\right)}{\sum_z\exp\left(\frac{\epsilon u(\x, z)}{2\Delta(u)}\right)}\\
%     =& \exp(\epsilon)
% \end{align*}
% \end{proof}




\section{Statistical and Practical Considerations}\label{sec:discussion}

\noindent\textbf{Unbiasedness of projection algorithms}
The projection algorithms proposed in this paper, be they Laplace or Gaussian, are provably \emph{unbiased} due to their additive construction. In fact, we have the following result.
\begin{corollary}\label{cor:unbiasedness}
Any mechanism of the form $\mathcal{M}(\x):=A(\x)+\Pi_{\mathcal{N}}\mathbf{e}$ as defined in Corollary~\ref{cor:projection},  where ${\bf e}$ is random noise with $\E\left({\bf e}\right) = 0$, is unbiased in the sense that
\begin{equation*}
\E\left[\mathcal{M}({\bf x}) \mid  A({\bf x})\right] = A\left({\bf x}\right).    
\end{equation*}
\end{corollary}
Corollary~\ref{cor:unbiasedness} stands because the conditional expectation of its noise component, $\E\left[\Pi_{\mathcal{N}}{\bf e} \mid A({\bf x})\right]$, is zero, due to the independence of ${\bf e}$ from $A({\bf x})$, and the nature of the projection operation. All projection mechanisms proposed in this paper are of this type, hence are unbiased. As for the proposed extension algorithms, their purpose is to augment existing DP mechanisms in a way that satisfy mandated invariants, thus their unbiasedness hinge on the unbiasedness of the initial mechanism which they extend. For applications in which the data curator has the freedom to design the privacy mechanism from scratch, projection mechanisms are the recommended way to proceed. Indeed, both numerical demonstrations in Section~\ref{sec:example} applied to the county-level 2020 Census demonstration data and the spatio-temporal university campus data utilize the projection mechanisms, guaranteeing the unbiasedness of the sanitized data products under their respective invariant constraints. 


\noindent\textbf{Transparency and statistical intelligibility}
%Equivalence with Invariant Conditionalization 
%\fang{better place? 4.3? Gaussian? Other mechanisms closure property. pure or not pure}
%Unbiased and transparency%
%The construction of the invariant-respecting Gaussian mechanism has its special statistical significance.
%The invariant-respecting Gaussian mechanism in Definition~\ref{def:gaussian} 
% Mechanisms constructed via \Cref{cor:projection} carries a special advantage in terms of their statistical intelligibility. Gaussian mechanisms, in particular, further enjoy the  equivalence between projection and probabilistic conditioning. We defer the discussion on this matter to Section~\ref{sec:discussion}. 
Subspace differentially private additive mechanisms carry a special advantage when examined through the lens of downstream statistical analysis of the output query. All Gaussian and Laplace mechanisms examined in this paper (\cref{cor:projected_gaussian,cor:extended_gaussian,cor:projected_laplace,cor:extended_laplace,thm:sdp_corr_gaussian}), be they obtained via projection or extension, linearly combine the confidential query with a noise term that is publicly specified. Just like standard differential privacy, mechanisms of subspace differential privacy described in this paper are \emph{transparent} \citep{abowd2016economic}, a prized property that brought revolutionary change to the literature of statistical disclosure limitation by ridding obscure procedures. Moreover, the employed noise terms have probability distributions that are fully characterized and independent of the confidential query. This grants the mechanisms \emph{statistical intelligibility} \citep{gong2020congenial}, making the output query eligible for both analytical and simulation-based (such as bootstrap) statistical analysis and uncertainty quantification. 


% As a special case, if $M$ is the widely employed spherical Gaussian mechanism (to be defined in~\Cref{lem:gaussian}), the constructed $\mathcal{M}$ further enjoys an equivalence between the projection to, and the probabilistic conditioning on the invariant margin. This greatly facilitates principled downstream statistical analysis. We defer the discussion on this matter to \Cref{sec:discussion}. \jie{This paragraph is a bit early? maybe we should move it to section 3.3?}
%As alluded to after~\Cref{cor:projection}, 

In the special case that the original unconstrained differentially private mechanism is spherical Gaussian, defined in~\Cref{lem:gaussian}, the \goodprivacy mechanism resulting from projection produces a random query that is distributionally equivalent to that obtained via the standard probabilistic conditioning of the unconstrained mechanism, where the conditioning event is precisely the invariants that the curator seeks to impose. 

\begin{theorem}\label{thm:conditioning}
If the additive mechanism $M$ in~\Cref{cor:projection} is spherical Gaussian as defined in~\Cref{lem:gaussian}, the corresponding modified mechanism $\mathcal{M}$ has a probability distribution equivalent to the distribution of $M$ conditional on the invariant being true. That is,
$$
\mathcal{M}(\x)  \overset{d}{=} {M}(\x) \mid C{M}(\x)=CA(\x).$$
\end{theorem}

The proof of \Cref{thm:conditioning} is given in Appendix~\ref{app:spherical-proof}.  The equivalence with conditionalization is particularly valuable for Bayesian inference based on the privatized query, as the analyst may coherently utilize all available information.  We note here however, that \Cref{thm:conditioning} results from unique properties of the spherical Gaussian distribution. In general, the projection operation aligns closer with marginalization, and cannot produce the equivalent distribution as conditionalization. Nevertheless, the happy statistical consequence of \Cref{thm:conditioning} may still be widely impactful, thanks to the ubiquity of the spherical Gaussian mechanism.


%\robin{LET'S MOVE THIS TO APPENDIX - This proof reads longer than I thought. Maybe we can move this instead.}

% downstream statistical analysis, in that the distribution of their output query is equivalent to that obtained via statistical conditioning of an otherwise unrestricted differentially private query, on the hard constraint given by the invariant.

%the The probabilistic distribution of according to statistical conditioning of available evidence as given by the invariant. 

% \begin{theorem}
% The Gaussian Mechanism with linear equality invariant in Definition~\ref{def:gaussian} has a probability distribution that is the conditional distribution of the unconstrained Gaussian Mechanism in Definition~\ref{def:gaussian0} conditional on the invariant being true. That is,
% \begin{equation}\label{eq:conditional}
% M\left({\bf x}\right) \quad \overset{d}{=} \quad M^{*}\left({\bf x}\right)\mid CM^{*}\left({\bf x}\right)=CA{\bf x}.	
% \end{equation}
% \end{theorem}
% \robin{I haven't rewritten this bit below to flush out the flow, but we may or may not keep this bit depending on space...}
% {\color{blue}
% It seems like given any \goodprivacy mechanism $\mathcal{M}$, we can always find a differentially private mechanism $M$ such that the conditional distribution $M|(CM(\x) = CA\x) = \mathcal{M}$.  Specifically, we can decompose the query $A$ into $\Pi_\mathcal{N}A$ and $\Pi_\mathcal{R}A$ and design two $(\epsilon/2, \delta/2)$-differential private mechanisms for each query and compose their reports. 
% }

% {\color{blue} 
% Note that ${\bf e}\overset{d}{=}{\bf u}\mid C{\bf u}={\bf 0}$. That
% is, the distribution in \eqref{eq:error_distribution} is the conditional
% distribution of ${\bf u}$ (the additive error of the unconstrained
% mechanism) given $C{\bf u}=0$. [Note that the cleaness of the derivation hinges on the fact that the constrained mechanism uses an error distribution that is independent of the confidential query value.]

% It is also worth noting that the covariance
% matrix $\Sigma_{C}$ has a special interpretation in the linear regression
% context. It is precisely the covariance matrix of the residual vector
% for a multiple linear regression with design matrix $C^{\top}$. See
% Models as Constraints section for more on this.}


% {\color{blue} There exists an equivalence between this approach and the conditional distribution approach as described in Section 2. Here, we're directly constructing distribution of the noise terms within the linear subspace, whereas in Section 2, the distribution is a conditional distribution deduced from an unconstrained mechanism. There must be quite some connection between the noise component $Q_{C}{\bf u}$ here, and the term $\Gamma {\bf u}$ in \eqref{eq:constrained-normal}. Although, the two are not necessarily identical in distribution, because the scale parameters was either deduced (in the former case) or directly picked (here). This needs further verification.}

\noindent\textbf{Implementation: distributed privatization}
In local differential privacy, we consider the identity mapping as the query function $A$, and the private mechanism directly infuses entry-wise noise into the entire confidential dataset before releasing it to the public. The confidential dataset, $\x$, is often gathered by a number of local agents -- nodes, sensors, survey workers -- each responsible for one (or more) entries of $\x$. Distributed privatization can be valuable in local differential privacy, as it ensures individual data contributors' information is protected the moment it leaves the local agent. 

For all additive subspace differentially private mechanisms proposed in this work, distributed privatization may be achieved,  if the local agents are capable of simulating the same noise component. The synchronized simulation can be implemented --  hardware permitting -- by sharing a common seed across the different local sensors or workers. An instance of distributed privatization is spelled out in Algorithm~\ref{alg:distributed} in Appendix~\ref{app:distributed}, which works for arbitrary linear equality invariant $C$.

%\fang{Deferred to supplementary material:When invariants are in place, the feasibility of distributed privatization may be counter-intuitive, because invariants typically induce dependence among entries of the private query. The key here is that for additive mechanisms that impart linear equality invariants, the noise that each local agent infuses does not depend on the confidential $\x$ at all. With a shared seed, every agent can generate the same noise vector ($\mathbf{e}$ in Algorithm~\ref{alg:distributed}), and carry out their privatization task in isolation from others.}
%The only requirement is that a common seed is shared across all local agents for noise simulation. , we agree that the insufficiency of using  can be a real technical challenge to the distributization of the proposed privatization framework. We will revise the phrasing of the requirement that 




%{\color{blue} Finally, the addition of each agent's report is \goodprivacy, because addition is commutative. }\robin{I don't understand this statement...}

%The proposed mechanism supports distributed privatization. 



%This pertains to the special case of local differential %privacy, in which
%and the query function $A$ is the identity mapping, and In this context, 
%\eqref{eq:additive}
%Notice that all our mechanisms (Gaussian, Laplace, and $k$-norms) are additive and can easily be converted to distributed mechanisms.   


% , and the output would be In particular, the following meta-algorithm apply to \fang{reference}, and Laplace mechanisms in \Cref{lem:laplace}. \robin{broken reference} The meta-algorithm below distributes the privatization task to each agent. Every agent carries out the privatization locally, while ensuring that the aggregated privatized data ${\bf y}$ satisfies the global invariant constraint in \Cref{def:invariant}.









\section{ Numerical Examples}\label{sec:example}


%\jie{one thought: should we put discussion earlier than numerical examples? also maybe we can shorten the numerical example to one sentence or so (for saving space) as most details are in the appendix anyway.}

% \noindent\textbf{2020 Census demonstration data}
% We consider the publication of induced subspace differentially private county-level Census population counts, subject to the invariant of state population size, using the November 2020 vintage privacy-protected demonstration files curated by IPUMS NHGIS \cite{ipums2020das}. Right panel of Figure~\ref{fig:census_trend} showcases the county-level errors from ten runs of the projected Laplace $(\epsilon,0)$-induced subspace differentially private mechanism of \Cref{cor:projected_laplace}, applied to the counties of Illinois arranged in increasing true population sizes.  Compared with the DAS errors (red squares) which show a clear negative bias trend, the proposed mechanism is provably unbiased, due to its additive errors being projected from unbiased and unconstrained random variables. On the other hand, these errors span a similar scale compared to the DAS errors. Details of the implementation are given in Appendix~\ref{app:example}, and results for additional states in Figure~\ref{fig:census_sdp_county2}.  


%\noindent\textbf{2020 Census demonstration data}

\subsection{2020 Census Demonstration Data}

We consider the publication of induced subspace differentially private county-level Census population counts, subject to the invariant of state population size, using the November 2020 vintage privacy-protected demonstration files curated by IPUMS NHGIS \cite{ipums2020das}. These data files link together the original tables from the 2010 Census Summary Files (CSF), here treated as the confidential values, and the trial runs of the Census Bureau's 2020 Disclosure Avoidance System (DAS) applied to the CSF. All these datasets are publicly available at the cited source. For our demonstration, the privacy loss budget is set to accord exactly to the Census Bureau's specification, with $\epsilon = 0.192 = 4 \text{ (total)} \times 0.16 \text{ (county level)} \times 0.3 \text{ (population query)}$. 

Right panel of Figure~\ref{fig:census_trend} showcases the county-level errors from ten runs of the projected Laplace $(\epsilon,0)$-induced subspace differentially private mechanism of \Cref{cor:projected_laplace}, applied to the counties of Illinois arranged in increasing true population sizes.  Compared with the DAS errors (red squares) which show a clear negative bias trend, the proposed mechanism is provably unbiased, due to its additive errors being projected from unbiased and unconstrained random variables. On the other hand, these errors span a similar scale compared to the DAS errors. Figure~\ref{fig:census_sdp_county2} in Appendix~\ref{app:example} shows the application of the projected Laplace $(\epsilon,0)$-induced subspace differentially private mechanism to an additional ten states, for which the TopDown algorithm incurred decidedly negatively biased errors. Details of how these states were identified are given in Section~\ref{sec:intro}. We can make similar observations from Figure~\ref{fig:census_sdp_county2} about the errors from the proposed mechanism as we did from Figure~\ref{fig:census_trend}, including their unbiasedness yet a similar error scale compared to the DAS errors.






% On the right hand side of Figure~\ref{fig:census_trend}, the boxplots showcase the county-level errors from ten runs of the projected Laplace $(\epsilon,0)$-induced subspace differentially private mechanism of \Cref{cor:projected_laplace}, applied to the county populations of Illinois. From left to right, the counties are arranged in increasing true population sizes. The privacy loss budget $\epsilon$ is set to $0.192 = 4 \text{ (total)} \times 0.16 \text{ (county level)} \times 0.3 \text{ (population query)}$, according to Census Bureau's specification of the November 2020 vintage.

% Compared with the DAS errors (red squares) which show a clear negative bias trend, the induced subspace differentially private mechanism is provably unbiased, due to its additive errors being the projection of unbiased and unconstrained random variables. The errors also span a similar scale compared to the DAS errors. Appendix~\ref{app:example} shows the application of the induced subspace differentially private Laplace mechanism to an additional ten states for which the TopDown algorithm incurred decidedly negatively biased errors. Similar observations -- i.e. unbiasedness and similar error scale -- can be made.

%\noindent\textbf{Spatio-temporal dataset}

% We consider the publication of tabulated hourly time series for $14$ groups of fully anonymized individuals who spent some amount of time at any of the $20$ locations on a large university campus (Tsinghua University) in a single day~\cite{sui2016characterizing}. The invariants are the total number of person-hours spent at each location every hour from all groups, as well as that by every group over 24 hours. The query is in total $6720$ dimensional, subject to a $740$-dimensional linear constraint. We apply the projection Gaussian mechanism in \Cref{cor:projected_gaussian}. The mechanism is again provably unbiased, although the error exhibit a slight loss of scale due to the abundance of linear constraints imposed. Over 50 repetitions of the mechanism, the median standard deviation of the elementwise additive errors is $0.88$ (relative to one unit), with $5\%$ and $95\%$ quantiles at $(0.86, 0.91)$ respectively. Details of the implementation can be found in Appendix~\ref{app:example}, with results displayed in Figure~\ref{fig:tsinghua}.

\subsection{Spatio-temporal Dataset}

We consider the publication of time series derived from WiFi log data on connections of mobile devices with nearby access points from a large university campus (Tsinghua University)~\cite{sui2016characterizing} consisting of $3243$ fully anonymized individuals and the top $20$ most popularly visited buildings in one day. \footnote{Data was collected under the standard consent for Wifi access on university campus. Interested reader may contact the authors of \cite{sui2016characterizing} to inquire access to the dataset.} The raw data recorded whether an individual appears in each of the building in each of the hours on one day. The data were tabulated into hourly time series for $14$ clusters of individuals obtained through simple $K$-means, to represent hypothetical group memberships with distinct travel patterns. 

The invariants we consider are of two types, motivated by needs for building management, energy-control, and group activity scheduling: 1) the total number of person-hours spent at each building every hour from all groups, and 2) the total number of person-hours spent at each building by every group over 24 hours. The query under consideration is $14\text{ (groups)}\times 24\text{ (hours)}\times 20\text{ (location)} = 6720$ dimensional, subject to a $(24 + 14 - 1)\times 20 = 740$-dimensional linear constraint. 
	
We apply the projection Gaussian mechanism in \Cref{cor:projected_gaussian}.
%, where for simplicity of comparison, the scale of the elementwise Gaussian noise is set to $1$. 
The comparison of confidential data and one run of the induced subspace differentially private mechanism is displayed in Figure~\ref{fig:tsinghua}. 
%The mechanism is provably unbiased, and exhibits some loss of scale due to the numerous linear constraints imposed. Over 50 repetitions of the mechanism, the median standard deviation of the elementwise additive errors is $0.88$, with $5\%$ and $95\%$ quantiles at $(0.86, 0.91)$ respectively.
The mechanism is again provably unbiased, although the errors exhibit a slight loss of scale due to the numerous linear constraints imposed. Over 50 repetitions of the mechanism, the median standard deviation of the elementwise additive errors is $0.88$ (relative to one unit), with $5\%$ and $95\%$ quantiles at $(0.86, 0.91)$ respectively. Results of the simulation are displayed in Figure~\ref{fig:tsinghua} of Appendix~\ref{app:example}.


% We used the WiFi log data on connections of mobile devices with nearby WiFi access points from a large university campus (Tsinghua University)~\cite{sui2016characterizing}, consisting of $3243$ fully anonymized individuals and the top $20$ most popularly visited buildings in one day. The raw data recorded whether an individual appears in each of the building in each of the hours on one day. The data were tabulated into hourly time series for $14$ clusters of individuals obtained through simple $K$-means, to represent hypothetical group memberships with distinct travel patterns. The invariants we consider are of two types, motivated by needs for building management, energy-control, and group activity scheduling: 1) the total number of person-hours spent at each building every hour from all groups, and 2) the total number of person-hours spent at each building by every group over 24 hours. 
% Thus, the query we consider is $14\text{ (groups)}\times 24\text{ (hours)}\times 20\text{ (buildings)} = 6720$ dimensional, subject to a $740$-dimensional linear constraint. 
	
% We apply the projection Gaussian mechanism in \Cref{cor:projected_gaussian}, where for simplicity of comparison next, the scale of the elementwise Gaussian noise is set to $1$. The comparison of confidential data and one run of the induced subspace differentially private mechanism is displayed in Figure~\ref{fig:tsinghua} in Appendix~\ref{app:example}. The mechanism is again provably unbiased, although the error exhibit a slight loss of scale due to the abundance of linear constraints imposed. Over 50 repetitions of the mechanism, the median standard deviation of the elementwise additive errors is $0.88$, with $5\%$ and $95\%$ quantiles at $(0.86, 0.91)$ respectively.
% 

% \begin{figure}
% %\includegraphics[width = \textwidth]{figs/sdp_error_by_county_26}
% \includegraphics[angle=90,origin=c,height= .8\textheight]{figs/tsinghua_student_hours_kmeans.pdf}
% \caption{\label{fig:tsinghua}. }	
% \end{figure}


% \section{Comparison with other privacy}

% \robin{I will take care of this section in Sec 1 (intro) as a literature review.}

% \subsection{other privacy}
% \fang{conditional differential privacy}
% \fang{Bayesian inference}
% \fang{Pufferfish, induced neighborhood, and linear subspace constraints}



\section{Conclusion and Future Work} \label{sec:conclusion}

In this paper, we proposed the concept of subspace differential privacy to make explicit the mandated invariants imposed on private data products, and discussed the projection and extension designs of induced differentially private mechanisms. The invariants we consider are in the form of linear equalities, including sums and contingency table margins as often encountered in applications including the U.S. Decennial Census and spatio-temporal datasets.

An important type of invariants not addressed in this paper are inequalities, such as nonnegativity and relational constraints (e.g. the population size must be larger or equal to the number of households in a geographic area). However, we note that an important premise to the unbiasedness achieved by subspace differentially private mechanisms, as discussed in Section~\ref{sec:discussion}, is that the mechanism admits equality invariants only. If inequality invariants must be imposed, unbiased privacy mechanisms can be inherently difficult to design. As \citet{DBLP:journals/corr/abs-2010-04327} discussed, the bias induced by projection-type post-processing of noisy measurements is attributable to the non-negativity constraints imposed on them. This raises the question of the appropriateness of inequality invariants on the sanitized output, if unbiasedness is simultaneously required. 


Also not considered are invariants for binary and categorical attributes, taking values in a discrete space. These invariants differ from real-valued linear equality invariants, because in general they cannot be realized by an additive mechanism with a noise term independent of the confidential data value. While the notion of subspace differential privacy can be extended to these cases, the design of accompanying privacy mechanisms that also enjoy good statistical and implementation properties remains a subject of future research.

%\clearpage

% and integer requirements

% ``soft'' invariants, such as inequalities (e.g., the electricity usage should be a positive number) and integral requirements (e.g., binary attributes).  
